RCPS: Rectified Contrastive Pseudo Supervision for Semi-Supervised Medical Image Segmentation

Medical image segmentation methods are generally designed as fully-supervised to guarantee model performance, which require a significant amount of expert annotated samples that are high-cost and laborious. Semi-supervised image segmentation can alleviate the problem by utilizing a large number of unlabeled images along with limited labeled images. However, learning a robust representation from numerous unlabeled images remains challenging due to potential noise in pseudo labels and insufficient class separability in feature space, which undermines the performance of current semi-supervised segmentation approaches. To address the issues above, we propose a novel semi-supervised segmentation method named as Rectified Contrastive Pseudo Supervision (RCPS), which combines a rectified pseudo supervision and voxel-level contrastive learning to improve the effectiveness of semi-supervised segmentation. Particularly, we design a novel rectification strategy for the pseudo supervision method based on uncertainty estimation and consistency regularization to reduce the noise influence in pseudo labels. Furthermore, we introduce a bidirectional voxel contrastive loss to the network to ensure intra-class consistency and inter-class contrast in feature space, which increases class separability in the segmentation. The proposed RCPS segmentation method has been validated on two public datasets and an in-house clinical dataset. Experimental results reveal that the proposed method yields better segmentation performance compared with the state-of-the-art methods in semi-supervised medical image segmentation. The source code is available at https://github.com/hsiangyuzhao/RCPS.

==> data/pancreas_comparison.tex <==
\begin{table*}[]
\centering
\caption{Performance comparison on the pancreas-CT dataset. The best two results are highlighted in bold.}
\label{table:pancreas}
\setlength{\tabcolsep}{3mm}{
\begin{tabular}{@{}cccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Scans Used}} & \multicolumn{3}{c}{\textbf{Metrics}} \\ 
\cmidrule(l){2-6} 
                        & Labeled         & Unlabeled    & DSC(\%)$\uparrow$    & HD95{\scriptsize (voxel)}$\downarrow$   & ASD{\scriptsize (voxel)}$\downarrow$    \\
                        \midrule
Fully-Supervised        & 6   (10 \%)     & 0            & 55.20   & 30.62   & 10.54   \\
Fully-Supervised        & 12   (20 \%)    & 0            & 72.38   & 20.64   & 5.41    \\
Fully-Supervised        & 62   (All)      & 0            & 83.89   & 5.08    & 2.00    \\
\midrule
\midrule
UA-MT \cite{yu2019uncertainty}   & 6   (10 \%)     & 56           & 66.44   & 17.04   & 3.03    \\
SASSNet \cite{li2020shape}  & 6   (10 \%)     & 56           & 68.97   & 18.83   & \textbf{1.96}    \\
DTC \cite{luo2021dualtask}       & 6   (10 \%)     & 56           & 66.58   & \textbf{15.46}   & 4.16    \\
URPC  \cite{luo2021efficient}    & 6   (10 \%)     & 56           & \textbf{73.53}   & 22.57   & 7.85    \\
MC-Net+ \cite{wu2022mutual}   & 6   (10 \%)     & 56           & 70.00   & \textbf{16.03}   & 3.87    \\
% Multi-scale MC-Net+  \cite{wu2022mutual}  & 6   (10 \%)    & 60           & 74.01   & 12.59    & \textbf{3.34}    \\
\textbf{Ours}           & 6   (10 \%)     & 56           & \textbf{76.62}   & 16.32   & \textbf{3.01}    \\
\midrule
\midrule
UA-MT  \cite{yu2019uncertainty}  & 12   (20 \%)    & 50           & 76.10   & 10.84   & 2.43    \\
SASSNet \cite{li2020shape} & 12   (20 \%)    & 50           & 76.39   & 11.06   & \textbf{1.42}    \\
DTC  \cite{luo2021dualtask}      & 12   (20 \%)    & 50           & 76.27   & 8.70    & 2.20    \\
URPC  \cite{luo2021efficient}   & 12   (20 \%)    & 50           & \textbf{80.02} & \textbf{8.51} & 1.98    \\
MC-Net+  \cite{wu2022mutual}  & 12   (20 \%)    & 50           & 79.37   & 8.52    & \textbf{1.72}    \\
% Multi-scale MC-Net+  \cite{wu2022mutual}  & 12   (20 \%)    & 50           & 80.59   & 6.47   & \textbf{1.74}    \\
\textbf{Ours}           & 12   (20 \%)    & 50           & \textbf{81.59} & \textbf{7.50} & 2.03    \\ \bottomrule
\end{tabular}}
\end{table*}
